Soft Q Network

Deep Q Network (DQN) is a very successful algorithm, yet the inherent problem of reinforcement learning, i.e. the exploit-explore balance, remains. In this work, we introduce entropy regularization into DQN and propose SQN. We find that the backup equation of soft Q learning can enjoy the corrective feedback if we view the soft backup as policy improvement in the form of Q, instead of policy evaluation. We show that Soft Q Learning with Corrective Feedback (SQL-CF) underlies the on-plicy nature of SQL and the equivalence of SQL and Soft Policy Gradient (SPG). With these insights, we propose an on-policy version of deep Q learning algorithm, i.e. Q On-Policy (QOP). We experiment with QOP on a self-play environment called Google Research Football (GRF). The QOP algorithm exhibits great stability and efficiency in training GRF agents.

==> defs.tex <==
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\lcmt}[1]{{\footnotesize\textcolor{red}{#1}}\\}
\newcommand{\todo}[1]{\cmt{(TODO: #1)}}


\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\etal}{et al.\ }
\newcommand{\cf}{cf.}

% Math operators and functions
\newcommand{\E}[2]{\operatorname{\mathbb{E}}_{#1}\left[#2\right]}
\newcommand{\Eleft}[2]{\operatorname{\mathbb{E}}_{#1}\left[#2\right.}
\newcommand{\Eright}[2]{\left.#2\right.}
\newcommand{\EEE}{\mathbb{E}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\density}{p}
\newcommand{\proposal}{q}  % proposal distribution
\newcommand{\target}{p}  % target distribution
\newcommand{\prop}{P}
%\newcommand{\kl}{\mathrm{D_{KL}}}
\newcommand{\kl}[2]{\mathrm{D_{KL}}\left(#1\;\middle\|\;#2\right)}
\newcommand{\entropy}{\mathcal{H}}
\newcommand{\ent}{\mathcal{H}}
\newcommand{\tr}{\mathrm{tr}}

% Constant matrices and vectors.
\newcommand{\ones}{\boldsymbol{1}}
\newcommand{\eye}{\boldsymbol{I}}
\newcommand{\zeros}{\boldsymbol{0}}

% Other helpers
\newcommand{\voidarg}{{\,\cdot\,}}


% MDP
\newcommand{\sspace}{\mathcal{S}}
\newcommand{\aspace}{\mathcal{A}}
% \newcommand{\xspace}{\mathcal{X}}
\newcommand{\latspace}{\mathcal{H}}
\newcommand{\state}{\mathbf{s}}
\newcommand{\sz}{{\state_0}}
\newcommand{\stm}{{\state_{t-1}}}
\newcommand{\st}{{\state_t}}
\newcommand{\sti}{{\state_t^{(i)}}}
\newcommand{\sT}{{\state_T}}
\newcommand{\stp}{{\state_{t+1}}}
\newcommand{\stpi}{{\state_{t+1}^{(i)}}}
\newcommand{\pdyn}{\density}
% \newcommand{\pdyn}{\density_\state}
\newcommand{\horizon}{T}
\newcommand{\hm}{{T-1}}
\newcommand{\action}{\mathbf{a}}
\newcommand{\az}{{\action_0}}
\newcommand{\atm}{{\action_{t-1}}}
\newcommand{\at}{{\action_t}}
\newcommand{\ati}{{\action_t^{(i)}}}
\newcommand{\atj}{{\action_t^{(j)}}}
\newcommand{\attildej}{{\tilde{\action}_t^{(j)}}}
\newcommand{\atij}{{\action_t^{(i,j)}}}
\newcommand{\atp}{{\action_{t+1}}}
\newcommand{\aT}{{\action_T}}
\newcommand{\atk}{{\action_t^{(k)}}}
\newcommand{\aTm}{\action_{\horizon-1}}
\newcommand{\opt}{^*}
\newcommand{\obs}{\mathbf{o}}
\newcommand{\oz}{\obs_0}
\newcommand{\ot}{\obs_t}
\newcommand{\otp}{\obs_{t+1}}
\newcommand{\urv}{\mathbf{u}}

\newcommand{\latent}{\mathbf{h}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\x}{\mathbf{x}}

\newcommand{\optim}{\mathcal{O}}
\newcommand{\optimt}{\optim_t}
\newcommand{\optimtp}{\optim_{t+1}}
\newcommand{\optimT}{\optim_T}


% o

% Trajectories
\newcommand{\traj}{\tau}
\newcommand{\ptraj}{\density_\traj}
\newcommand{\visits}{\rho}  % Discounted visittation frequency

% Rewards
\newcommand{\reward}{r}
\newcommand{\rz}{\reward_0}
\newcommand{\rt}{\reward_t}
\newcommand{\rti}{\reward^{(i)}_t}
\newcommand{\rmin}{r_\mathrm{min}}
\newcommand{\rmax}{r_\mathrm{max}}
\newcommand{\return}{\eta}

% Optimality


% Value and Q function
\newcommand{\V}{V}
\newcommand{\Vsoft}{V_\mathrm{soft}}
\newcommand{\Vsoftpolicy}{\Vsoft^\policy}
\newcommand{\Vsoftpolicyold}{\Vsoft^{\policyold}}
\newcommand{\Vsoftparams}{V_\mathrm{soft}^\qparams}
\newcommand{\Vhatsoftparams}{\hat V_\mathrm{soft}^\qparams}
\newcommand{\Vhatsoft}{\hat V_\mathrm{soft}}
\newcommand{\Vhard}{V^{\dagger}}
\newcommand{\Vsofter}{V_\mathrm{softer}}
\newcommand{\Vsofterpolicy}{\Vsofter^\policy}
\newcommand{\Q}{Q}
\newcommand{\Qsoft}{Q_\mathrm{soft}}
\newcommand{\Qsoftpolicy}{\Qsoft^\policy}
\newcommand{\Qsoftpolicyold}{\Qsoft^{\policyold}}
\newcommand{\Qsoftparams}{Q_\mathrm{soft}^\qparams}
\newcommand{\Qsofter}{Q_\mathrm{softer}}
\newcommand{\Qsofterpolicy}{\Qsofter^\policy}
\newcommand{\Qhatsoft}{\hat Q_\mathrm{soft}}
\newcommand{\Qhatsoftparams}{\hat Q_\mathrm{soft}^{\bar\qparams}}
\newcommand{\Qhard}{Q^{\dagger}}
\newcommand{\A}{A}
\newcommand{\Asoft}{A_\mathrm{soft}}
\newcommand{\Asoftparams}{A_\mathrm{soft}^\qparams}
\newcommand{\Ahatsoft}{\hat A_\mathrm{soft}}

% EBM
\newcommand{\energy}{\mathcal{E}}

% Policy and params
\newcommand{\policy}{\pi}
\newcommand{\policyold}{{\policy_\mathrm{old}}}
\newcommand{\policynew}{{\policy_\mathrm{new}}}
\newcommand{\policynewa}{{\policy_\mathrm{nextnew}}}
\newcommand{\policyme}{\pi_\mathrm{me}}
\newcommand{\policyopt}{{\policy^*}}
\newcommand{\paramsz}{{\theta_0}}
\newcommand{\params}{\theta}
\newcommand{\paramsi}{{\theta_i}}
\newcommand{\paramsip}{{\theta_{i+1}}}
\newcommand{\softpolicy}{{\policy_\mathrm{soft}}}
\newcommand{\hardpolicy}{{\policy^{\dagger}}}
\newcommand{\pparams}{{\phi}}   % policy parameters
\newcommand{\qparams}{{\theta}}   % q function parameters
\newcommand{\eparams}{{\phi}}   % energy function params
\newcommand{\vparams}{{\psi}}   % energy function params
\newcommand{\vtargetparams}{{\bar\psi}}   % energy function params
\newcommand{\qtargetparams}{{\bar\theta}}   % q function parameters

% \newcommand{\policy}{{\pi_\params}}

% Policy gradient
\newcommand{\pgparams}{\phi}

% Losses
\newcommand{\pgloss}{J_\mathrm{PG}}
\newcommand{\qloss}{J_\Q}  % Bellman error loss (Q function loss).
\newcommand{\aloss}{J_\A}  % Bellman error loss on advantage.
\newcommand{\ploss}{J_\policy}  % Stein error loss (policy loss).



% EBM
\newcommand{\temp}{\alpha}  % temperature

% Stein method
\newcommand{\RKHSball}{\mathcal{F}}
\newcommand{\kernel}{\kappa}
%\newcommand{\sample}{\omega}  % generic sample
%\newcommand{\samplek}{\omega^{(k)}}  % generic sample
\newcommand{\smpl}{\xi}  % generic sample
\newcommand{\smpli}{\xi^{(i)}}  % generic sample
\newcommand{\smplj}{\xi^{(j)}}  % generic sample
\newcommand{\smpltildej}{\tilde{\xi}^{(j)}}  % alternative generic sample
\newcommand{\smplij}{\xi^{(i,j)}}  % generic sample






% ----- old -------


% losses
\newcommand{\loss}{\eta}
\newcommand{\lossi}{\loss_i}
\newcommand{\lossip}{\loss_{i+1}}
\newcommand{\meloss}{\loss_\mathrm{me}}

% Random variables.
\newcommand{\bopt}{\mathcal{O}}  % Binary random variable for optimality.
\newcommand{\boptt}{\bopt_t}  % Binary random variable for optimality.
\newcommand{\sinit}{\state_0}
%\newcommand{\st}{{\state_t}}
% \newcommand{\stp}{\state_{t+1}}
%\newcommand{\traj}{\tau}







% Policy.
\newcommand{\muat}{\boldsymbol \mu_{\at}}
\newcommand{\sigat}{\boldsymbol\Sigma_{\at}}

% Distributions.
%\newcommand{\dist}{p}
\newcommand{\dyndist}{p}
% \newcommand{\policy}{\pi_\theta}
\newcommand{\gauss}{\mathcal{N}}


% Other.
\newcommand{\vlb}{\mathcal{L}}
\newcommand{\const}{\mathrm{const}}

\newcommand{\inv}{^{-1}}
\newcommand{\T}{^\mathsf{T}}


%\DeclareMathOperator{\E}{\mathbb{E}}

% Spaces.
%\newcommand{\sspace}{\mathcal{S}}
%\newcommand{\aspace}{\mathcal{A}}
%\newcommand{\sspace}{\reals^d}
%\newcommand{\aspace}{\reals^p}
\newcommand{\rkhs}{\mathcal{H}^d}
\newcommand{\reals}{\mathbb{R}}

% Kernels.
%\newcommand{\kernel}{\kappa}
\newcommand{\rbf}{\kernel_{\mathrm{rbf}}}
\newcommand{\sigker}{\boldsymbol \Sigma_\traj}


% \newcommand{\params}{\theta}
\newcommand{\discount}{\gamma}
\newcommand{\cost}{c}
\newcommand{\totcost}{J}
\newcommand{\klcost}{J_\mathrm{KL}}
